Strategy Complexity of Parity Objectives in Countable MDPs

We study countably infinite MDPs with parity objectives. Unlike in finite MDPs, optimal strategies need not exist, and may require infinite memory if they do. We provide a complete picture of the exact strategy complexity of $\varepsilon$-optimal strategies (and optimal strategies, where they exist) for all subclasses of parity objectives in the Mostowski hierarchy. Either MD-strategies, Markov strategies, or 1-bit Markov strategies are necessary and sufficient, depending on the number of colors, the branching degree of the MDP, and whether one considers $\varepsilon$-optimal or optimal strategies. In particular, 1-bit Markov strategies are necessary and sufficient for $\varepsilon$-optimal (resp. optimal) strategies for general parity objectives.

==> basics.tex <==
In order to show the existence of Markov (or 1-bit Markov) strategies, it suffices to show the existence of memoryless (or 1-bit) strategies in an MDP that is made acyclic by encoding a step counter in the state space.
This idea appears already in~\cite{KMST:ICALP2019} and can be stated as follows.

\begin{restatable}{lemma}{acyclicMarkov}
\label{lem:acyclic-Markov}
Let $\?C\subset \N$ be a finite set of colors and $k \in \nat$.

1.~Suppose that for every acyclic MDP and every finite set $\states_0$ of states, %
$\eps$-optimal strategies from $\states_0$
for $\cParity{\?C}$ can be chosen deterministic $k$-bit.
Then for every MDP and every finite set $\states_0$ of states, %
$\eps$-optimal strategies from $\states_0$ for $\cParity{\?C}$ can be chosen deterministic $k$-bit Markov.

2.~Suppose that for every acyclic MDP  and every finite set $\states_0$ of states
that have an optimal strategy,
optimal strategies from $\states_0$ for $\cParity{\?C}$ can be chosen deterministic $k$-bit.
Then for every MDP and every finite set $\states_0$ of states
that have an optimal strategy,
optimal strategies from $\states_0$ for $\cParity{\?C}$ can be chosen deterministic $k$-bit Markov.


\end{restatable}
\ignore{
\begin{proof}
Consider an  MDP $\mdp$ with states $\states$ and a given finite set
 of initial states $\states_0$. We transform it into an acyclic MDP $\mdp'$ by encoding a
step-counter into the states (i.e., the states of $\mdp'$ are
 $\states \times \N$), let $\coloring((\state, n)) \eqdef \coloring(\state)$
and consider the finite set of initial states $\states_0 \times \{0\}$.
By our assumption, there exists an $\eps$-optimal (resp.\ optimal)
deterministic $k$-bit strategy $\zstrat'$ for $\formula$ from
$\states_0 \times \{0\}$ in $\mdp'$.
We can transform $\zstrat'$ back into an optimal $\eps$-optimal
(resp.\ optimal for $\eps=0$) deterministic $k$-bit Markov
strategy $\zstrat$ for $\formula$ from $\states_0$ in the original MDP $\mdp$
by keeping the step-counter in the strategy $\zstrat$ instead of the states.
\end{proof}
}


By the following lemma, the strategy complexity of general Parity
objectives does not depend on the branching degree of the MDPs.
However, this does not hold for particular Parity objectives with a restricted
set of colors, since the construction introduces an extra color.

\begin{restatable}{lemma}{infbranchingtofinitebranching}
\label{lem:inf-branching-to-finite-branching}
Suppose that for every finitely branching acyclic MDP
and 
Parity objective,
$\eps$-optimal (resp.\ optimal) strategies
can be chosen
deterministic $1$-bit.

Then even for every infinitely branching acyclic MDP and
Parity objective,
$\eps$-optimal (resp.\ optimal) strategies
can be chosen
deterministic $1$-bit.
\end{restatable}
\ignore{
\begin{proof}
We encode an infinitely branching countable acyclic MDP $\mdp$ into a finitely
branching acyclic countable MDP $\mdp'$.
Every controlled state $x$ with infinite branching
$x \to y_i$ for all $i \in \N$ is replaced by a gadget
$x \to z_1, z_i \to z_{i+1}, z_i \to y_i$ for all $i \in \N$
with fresh controlled states $z_i$.
Infinitely branching random states with $x \step{p_i}{} y_i$ for all $i \in \N$
are replaced by a gadget $x \step{1}{} z_1, z_i \step{1-p_i'} z_{i+1}, z_i \step{p_i'} y_i$ for all
$i \in \N$, with fresh random states $z_i$ and suitably adjusted probabilities
$p_i'$ to ensure that the gadget
is left at state $y_i$ with probability $p_i$, i.e.,
$p_i' = p_i/(\prod_{j=1}^{i-1}(1-p_j'))$.
The fresh states are labeled with an unfavorable color that is smaller than
all other colors, e.g., $-1$.

We take an $\eps$-optimal (for $\eps \ge 0$, where the case $\eps=0$ means
optimal) deterministic 1-bit strategy
$\zstrat'$ for Parity from all states $\state \in \states_0$ in $\mdp'$.
We construct a 1-bit deterministic $\eps$-optimal strategy $\zstrat$
for $\mdp$ as follows.
Consider some state $x$ that is infinitely branching in $\mdp$
and its associated gadget in $\mdp'$.
Whenever a run in $\mdp'$ according to $\zstrat'$ reaches $x$ with some
memory value $\alpha \in \{0,1\}$ there exist
values $p_i$ for the probability that the gadget is left at state
$y_i$. Let $p \eqdef 1-\sum_{i\in \N} p_i$ be the probability that the gadget is
never left. (If $x$ is controlled then only one $p_i$ (or $p$) is nonzero,
since $\zstrat'$ is deterministic. If $x$ is random then $p=0$.)
Since $\zstrat'$ is deterministic, the memory updates are deterministic,
and thus there are values $\alpha_i' \in \{0,1\}$ such that whenever
the gadget is left at state $y_i$ the memory will be $\alpha_i'$.
We now define the behavior of the 1-bit deterministic strategy $\zstrat$ 
at state $x$ with memory $\alpha$ in $\mdp$.

If $x$ is controlled and $p\neq 1$ then $\zstrat''$ picks the successor state $y_i$ where
$p_i=1$ and sets the memory to $\alpha_i'$.
If $p=1$ then any run according to $\zstrat'$ that enters the gadget
does not satisfy the objective. Thus $\zstrat$ performs at least as
well in $\mdp$ regardless of its choice, e.g., pick successor $y_1$ and
$\alpha' = \alpha$.

If $x$ is random then $p=0$ and the successor is chosen according to the defined
distribution (which is the same in $\mdp$ and $\mdp'$)
and $\zstrat$ can only update its memory.
Whenever the successor $y_i$ is chosen, $\zstrat$ updates the memory to
$\alpha_i'$.

In states that are not infinitely branching in $\mdp$, $\zstrat$ does
exactly the same in $\mdp$ as $\zstrat'$ in $\mdp'$.

Since all states in the gadgets are labeled with color $-1$, $\zstrat$ performs
at least as well in $\mdp$ as $\zstrat'$ in $\mdp'$ and is thus
$\eps$-optimal from every $\state \in \states_0$.
\end{proof}
}

For ease of presentation, we will, instead of showing the existence of $1$-bit
strategies in an acyclic MDP $\mdp$, show the existence of MD strategies in the corresponding
\emph{layered} MDP $\?L(\mdp)$, which encodes the two memory modes into the
states by having two copies of $\mdp$ (called \emph{layers} $0$ and $1$). 
The transitions and probability functions, as well as whether a state is
randomized, and its (Parity) color, are lifted naturally.

\begin{definition}[Layered Systems] %
\label{def:layered}
  Given an MDP $\mdp=\mdptuple$ with coloring $\coloring:\states\to \cset$,
  we define the corresponding
  \emph{layered MDP} $\?L(\mdp)=(L,L_\zsymbol,L_\rsymbol, \transition, \probp)$
  with coloring $\coloring:L\to \cset$
  as follows.\footnote{The auxiliary controlled states in $(\states\x\hat{\states}\x\{0,1\})$
in \cref{def:layered} are used to let the controller choose the layer after observing the outcome of a
random transition. They have the same color as their successor.}
  \begin{enumerate}
      \item $L\eqdef (\states\x\{0,1\}) \cup (\states\x\hat{\states}\x\{0,1\})$ where
      $\hat{\states}\eqdef \{\hat{\state} \mid \state \in \states\}$.
    \item $\coloring((\state,i)) \eqdef \coloring(\state)$
        and $\coloring((\state,\hat{\state}',i)) \eqdef \coloring(\state')$.
    \item $L_\zsymbol \eqdef (\states_\zsymbol \x \{0,1\}) \cup (\states\x\hat{\states}\x\{0,1\})$.
    \item For $\state \in \states_\zsymbol$ and all $i,j \in \{0,1\}$ we have
          $(\state,i)\transition (\state',j)$ iff $\state\transition \state'$.
    \item For $\state \in \states_\rsymbol$ we have $\probp((\state,i)\transition (\state,\hat{\state}',i)) \eqdef
      \probp(\state\transition \state')$
      and $(\state,\hat{\state}',i)\transition (\state',j)$ for all $i,j \in \{0,1\}$.
  \end{enumerate}
  We call states $(s,i)$ and $(s,1-i)$
  (resp.\ $(\state,\hat{\state}',i))$ and $(\state,\hat{\state}',1-i)$)
  \emph{siblings}
and say that a set $B\subseteq L$ of states is \emph{closed} iff for every contained state it also contains its sibling.
For any set $B\subseteq L$ of states, let 
$\closure{B}$ denote its minimal closed superset.
Note that if $\mdp$ is acyclic then $\?L(\mdp)$ is also acyclic.
\end{definition}

A crucial feature of $\?L(\mdp)$ is that the controller can freely choose the
layer at every step, which corresponds to updating the memory bit when playing
in $\mdp$. If a strategy is fixed in a (non-closed) part of a layered MDP
then the controller might not be able to switch freely between layers
any more. However, while playing outside of the closure of the fixed subspace,
he can still freely choose layers.

The next lemma shows the correspondence between deterministic 1-bit strategies
in $\mdp$ and MD strategies in $\?L(\mdp)$.

\begin{restatable}{lemma}{proplayered}
\label{prop:layered}
Let $\mdp$ be an acyclic MDP with states $\states$, $\coloring$ be a coloring,
$\?L(\mdp)$
the corresponding acyclic layered MDP,
$\states_0\subseteq \states$,
and $\formula=\Parity{\coloring}$.

For every deterministic $1$-bit strategy $\inducedStrat{\updatefun}{\memconf_0}$ in $\mdp$
there is a corresponding MD strategy $\tau$ in $\?L(\mdp)$, and vice-versa,
such that for any initial state $\state_0 \in \states_0$ and
initial memory mode $\memconf_0 \in \{0,1\}$,
$
\probm_{\?L(\mdp),(\state_0,\memconf_0),\tau}(\formula) =
\probm_{\mdp,\state_0,\inducedStrat{\updatefun}{\memconf_0}}(\formula) 
$.
\end{restatable}


\begin{definition}[Bubbles, Fixings]
    \label{def-fix-bubb}
    Let $\mdp$ be an MDP with states $\states$, $R\subseteq \states$, $l\in\N$.
    The \emph{$l$-bubble} around $R$ is the set
    \[\bubblearound{\mdp}{R}{l}
    \eqdef\{s \mid \exists s_0\in R. \exists \tau. \probm_{\mdp,\state_0,\tau}(\eventually^{\leq l} s) > 0 \}\]
    of states that can be reached from $R$ in at most $l$ steps.
    
    If $\tau$ is an MD strategy in $\mdp$
    we write $\fixin{\mdp}{\tau,R}$ for the MDP
    obtained from $\mdp$ by fixing the strategy $\tau$ for all states in $R$.
    That is,
        $\fixin{\mdp}{\tau,R}\eqdef
        (\states,\zstates\setminus R,\rstates\cup R,\transition{},\probp') \subseteq \mdp$
        where $\probp'(r)\eqdef\tau(r)$ for all $r\in R$.
    We will simply write $\fixin{\mdp}{\tau}$ for $\fixin{\mdp}{\tau, \states}$,
    where $\tau$ is fixed everywhere,
    and 
    $\fixinbubble{\mdp}{\tau}{R}{l}\eqdef
    \fixin{\mdp}{\tau,\bubblearound{\mdp}{R}{l}}$
    that fixes $\tau$ in the $l$-bubble around $R$.
\end{definition}
Any bubble around a closed set $R\subseteq L$ is closed.

\input{safesets}


==> safesets.tex <==
\begin{restatable}[Safe sets]{definition}{defSafesets}
\label{def:safeset}
Let $\mdp=\mdptuple$ be an MDP,
$\formula$ be an objective,
$\zstrat$ an MD-strategy
and $\beta \in [0,1]$.
$$
\safesub{\mdp,\zstrat,\formula}{\beta} \eqdef \{\state \in \states \mid 
\probm_{\mdp,\state,\zstrat}(\formula) \ge \beta\},
$$
is the set of states from which $\zstrat$ attains at least probability~$\beta$
for objective $\formula$, and
$$
\safesub{\mdp,\formula}{\beta} \eqdef
\{\state \in \states \mid
\valueof{\mdp,\formula}{\state} \ge \beta\}
$$
is the set of states whose value for $\formula$ is at least $\beta$.
\end{restatable}


